Conflict-Driven XOR-Clause Learning (extended version)

Modern conflict-driven clause learning (CDCL) SAT solvers are very good in solving conjunctive normal form (CNF) formulas. However, some application problems involve lots of parity (xor) constraints which are not necessarily efficiently handled if translated into CNF. This paper studies solving CNF formulas augmented with xor-clauses in the DPLL(XOR) framework where a CDCL SAT solver is coupled with a separate xor-reasoning module. New techniques for analyzing xor-reasoning derivations are developed, allowing one to obtain smaller CNF clausal explanations for xor-implied literals and also to derive and learn new xor-clauses. It is proven that these new techniques allow very short unsatisfiability proofs for some formulas whose CNF translations do not have polynomial size resolution proofs, even when a very simple xor-reasoning module capable only of unit propagation is applied. The efficiency of the proposed techniques is evaluated on a set of challenging logical cryptanalysis instances.

==> ecsystem.tex <==
\section{The xor-reasoning module ``\ECsys''}
This chapter introduces the necessary elements of the second xor-reasoning
module presented in~\cite{LJN:ICTAI2011}. We refer to it as ``\ECsys{}-module''
where \ECsys{} stands for Equivalence Class based parity reasoning. The
aim is to avoid deriving unnecessary intermediate xor-clauses by keeping
track of equivalence classes of variables.

The inference rules of the \ECsys{}-deduction system are listed in
Fig.~\ref{fig:ECRules} by using a similar notation as with the \ECAIsys{} deduction system. The rules are defined only for xor-clauses with at most
three variables, but this limitation can be circumvented by splitting each
xor-clause with four or more variables into an equisatisfiable conjunction of
xor-clauses with at most three variables per xor-clause. This is done by
repeatedly applying the rewrite rule
$(x_1 \xor x_2 \xor \dots \xor x_n) \leadsto
 {(x_1 \xor x_2 \xor y)
  (\neg y \xor x_3 \xor x_4 \xor ... \xor x_n)}$,
where $y$ is a fresh variable not occurring in other clauses.
We define
\emph{\ECsys-derivation},
\emph{\ECsys-derivable} (denoted by $\psi \ECderiv C$),
\emph{\ECsys-refutation},
and
(cnf-compatible) cut for a non-input vertex in \ECsys-derivation
as in Sect.~\ref{Sect:ECAI}
except that in
an \ECsys-derivation a vertex may have more than two incoming edges.
%
The \TerUnRule{} and \ConflictRule{} rules propagate known equivalences,
producing either
(i) an unary clause if the equivalences force literals
in an original xor-clause to have the same/opposite value,
or
(ii) a conflict if the equivalences force a variable to have a value opposite to its value, i.e.~if $x \equiv {\neg x}$ should hold.


\begin{figure}
  \small
  \begin{tabular}{@{}c@{\quad}c@{\quad}c@{}}
    $\inferencerule{x}{x \XX \True}{\False}$
    &
    $\inferencerule{x \XX \parity{1}}{x \XX y \XX z \XX \parity{2}}{y \xor z \xor (\parity{1} \xor \parity{2} \xor \True)}$
    &
    $\inferencerule{x \XX \parity{1}}{x \XX y \XX \parity{2}}{y \xor (\parity{1} \xor \parity{2} \xor \top)}$
    \vspace{1mm}
    \\
    {\footnotesize (a) \UnConflictRuleP} &
    {\footnotesize (b) \TerBinRuleP} &
    {\footnotesize (c) \BinUnRuleP}
    \\
    \\
    \multicolumn{3}{@{}l@{}}{
      $\inferencerulen{{x_1 \XX x_2 \XX \parity{1} \XX \top}\quad\dots\quad{x_{n-1} \XX x_{n} \XX \parity{n-1} \XX \top} \quad {x_1 \XX x_n \XX y \XX \parity{}}}
      {y \xor (\parity{1} \xor \parity{2} \xor \dots \xor \parity{n-1} \xor \parity{})} $
      %
      %$\inferencerulen{{x_1 \XX x_2 \XX \parity{1} \XX \top} \quad  {x_2 \XX x_3 \XX \parity{2} \XX \top} \ \dots\  {x_{n-1} \XX x_{n} \XX \parity{n-1} \XX \top} \quad {x_1 \XX x_n \XX y \XX \parity{}}}
      %{y \xor (\parity{1} \xor \parity{2} \xor \dots \xor \parity{n-1} \xor \parity{})} $
    }
    %\vspace{1mm}
    \\
    \multicolumn{3}{@{}c}{\footnotesize (d) \TerUnRuleP}
    \\
    \\
    \multicolumn{3}{@{}l}{
    %$\inferencerulenc{{x_1 \XX x_2 \XX \parity{1} \XX \top} \quad {x_2 \XX x_3 \XX \parity{2} \XX \top} \ \dots\  {x_{n} \XX x_{1} \XX \parity{n} \XX \top}}
    %                 {\bot}
    %                 {\parity{1} \XX \parity{2} \XX \dots \XX \parity{n} {=} \top}$
    $\inferencerulenc{{x_1 \XX x_2 \XX \parity{1} \XX \top}\quad ...\quad {x_{n-1} \XX x_n \XX \parity{n-1} \XX \top} \quad {x_{n} \XX x_{1} \XX \parity{n} \XX \top}}
                     {\bot}
                     {\parity{1} \XX \dots \XX \parity{n} {=} \top}$
%    $\inferencerulen{{A_1 \XX A_2 \XX \parity{1}} \quad  {A_2 \XX A_3 \XX \parity{2}} \ \dots\  {A_{n} \XX A_{1} \XX \parity{n}} \quad  {\parity{1} \XX \parity{2} \XX \dots \XX \parity{n} \XX \top}}
%                   {\bot}$
                 }
    %\vspace{1mm}
    \\
    \multicolumn{3}{@{}c}{\footnotesize (e) \ConflictRuleP}
\end{tabular}  
  \caption{Inference rules of \ECsys; the symbols $x,x_i,y,z$ are all variables while the $\parity{i}$ symbols are constants $\False$ or $\True$.}%  
  \label{fig:ECRules}%
\end{figure}

\begin{example}
Assume a conjunction of xor-clauses $ \xorclauses = (a \X b \X c) \land
(a \X c \X d) \land (b \X d \X e)  $.
Figure~\ref{fig:derivations} shows a $\ECAIsys$-derivation and an $\ECsys$-derivation of $ \xorclauses 
\land (a) $. The literal $e$ is $\ECAIsys$-derivable on
$ \xorclauses \land (a) $; the xor-reasoning module returns
$e$ as a xor-implied literal on $\xorclauses$ after $a$ is given
as a xor-assumption.
The cnf-compatible cut 1 for the literal $e$ shows that 
$\xorclauses \land (a) \Models (e)$
and
thus ${\orclauses \land \xorclauses} \Models ({\neg a} \lor e)$,
i.e.~$({\neg a} \lor e)$ is a xor-explanation for $e$.
\label{ex:derivations}
\end{example}

\begin{figure}[h]
  \centering
  \begin{tabular}{cc}
  \includegraphics[width=.48\columnwidth]{subst-example1}
  &
\includegraphics[width=.48\columnwidth]{ec-example1}
\\
        \end{tabular}

  \caption{A $\ECAIsys$-derivation and an $\ECsys$-derivation}
  \label{fig:derivations}
\end{figure}

\subsection{Implementing with Equivalence Classes}
\newcommand{\Merge}[3]{\operatorname{merge}(#1,#2,#3)}


The \ECsys-system makes heavy use of binary xor-clauses,
    i.e., equivalences between literals.
%
To efficiently detect when \ECsys-rules are applicable,
the \ECsys-module maintains and manipulates
these equivalence classes of literals.
%
Formally, given a conjunction $\Psi$ of xor-clauses,
    an equivalence relation $\equiv$ on $\LitsOf{\Psi} \cup \Set{\False,\True}$
    is \emph{consistent} if
    (i)
      for all literals $l_1$ and $l_2$,
        $l_1 \equiv l_2$ implies ${\neg l_1} \equiv {\neg l_2}$
        and
        (ii) $A \not\equiv {\neg A}$ holds for each atom $A$.
        %
        A consistent equivalence relation can be characterized by
        listing half of its equivalence classes and omitting the dual ones;
        e.g., if ${\equiv}$ ``is'' $\Set{\Set{x,\neg y,\True},\Set{z}}$,
        then ${\neg x} \equiv \False$.
%
E.g.,
     $\Merge{\Set{\Set{\True,x,\neg y},\Set{z},\Set{w}}}{\neg x}{z} = 
       \Set{\Set{\True,x,\neg y,\neg z},\Set{w}}$.
%
A consistent equivalence relation \emph{represents}
a conjunction $\Psi$ of xor-clauses if
it is the finest consistent equivalence relation
such that (i) $l \equiv \True$ for each unary clause $l$ in $\Psi$,
     and
     (ii) $x \equiv {y \xor \parity{} \xor \True}$ for each binary xor-clause
     $x \xor y \xor \parity{}$ in $\Psi$.
     E.g.,
     $\Set{\Set{x,\neg y,\True},\Set{z}}$
     represents $(\neg y) \land (x \xor y) \land (z \xor y \xor x)$.
%
To build an \ECsys-derivation,
   knowledge of which literals are in the same equivalence class
   is not enough but one has to explain \emph{why} they are in the same class.
%
For this purpose we propose that the equivalence data structure is augmented
with an ``equivalence reason graph'' which records
the reasons for the equivalence class merges performed.
%
It turns out that with this structure there is no need to explicitly build
an \ECsys-derivation at all but xor-explanations can be computed
directly from it.
%
Formally,
    given a conjunction $\xorclauses$ of xor-clauses,
    an \emph{equivalence reason graph} over $\xorclauses$
    is an undirected, edge-labeled graph $G = \Tuple{V,E}$
    where
    (i) the vertex set is $V = \VarsOf{\xorclauses}\cup\Set{\True}$,
    and
    (ii) $E$ is an ordered set of labeled edges,
    i.e.~a sequence of disjoint elements over
    $W \times \Set{\False,\True} \times R$,
    where
    $W$ is the set of all 2-subsets of $V$,
    and
    $R$ is the set of unary and binary xor-clauses over $\VarsOf{\xorclauses}$
    augmented with a special symbol~$\Assump$.
    %
    For each labeled edge $\Tuple{\Set{v_1,v_2},\parity{},r} \in E$
    between $v_1$ and $v_2$,
    we may write $v_1 \Bcgedge{\parity{}}{r} v_2$,
    define the \emph{index} of the edge to be $i$ if it is the $i$th edge in $E$,
    and
    call the edge an \emph{equality edge} if $\parity{} = \False$ and
    a \emph{disequality edge} if $\parity{} = \True$.
    %
    Intuitively,
    an edge $v_1 \Bcgedge{\parity{}}{r} v_2$ denotes that
    ``$v_1 \xor v_2 = \parity{}$ holds because $r$ holds'',
    the case $r=\Assump$ denoting a xor-assumption.
    %
    A path
    ${v_1 \Bcgedge{\parity{1}}{r_1} v_2 \Bcgedge{\parity{2}}{r_2} ...
         \Bcgedge{\parity{n}}{r_n} v_{n+1}}$
         is a $\parity{}$-path if $\parity{} = \parity{1}\xor...\xor\parity{n}$.
         %
         The index of a path is the largest index of the edges in it.
         %

We now describe how the \ECsys-rules act on equivalence classes and
how reason graphs are built.
%
Let $\equiv$ be an equivalence class representing the original xor-clauses
$\xorclauses$ as well as
xor-assumptions and derived xor-clauses so far.
\begin{itemize}
\item
  If we make a xor-assumption $x \xor \parity{}$,
  then we
  (i) merge the classes of $\True$ and $x \xor \parity{}$, and
  (ii) add the edge $\True \Bcgedge{\parity{}}{\Assump} x$
  in the graph.
\item
  The \UnConflictRule{} and \ConflictRule{} rules are applicable when
  $\equiv$ is inconsistent:
  only in such a case there is a variable $x$
  for which $x \equiv {\neg x}$ holds.
\item
  The \TerBinRule{} rule is applicable when there is
  (i) a literal $x \xor \parity{1}$ such that
  $\True \equiv {x \xor \parity{1}}$ holds,
  and
  (ii) a xor-clause $x \XX y \XX z \XX \parity{2}$ in $\xorclauses$.

  When this rule is applied,
  (i) the equivalence classes of $y$ and $z \xor \parity{1} \xor \parity{2}$
  are merged, and
  (ii) the edge
  $y \Bcgedge{\parity{1} \xor \parity{2}}{x \xor \parity{1}} z$
  is added in the reason graph
  to record that $y$ and $z \xor \parity{1} \xor \parity{2}$
  are equivalent because $x \xor \parity{1}$ is true.
\item
  The rule \BinUnRule{} is implicitly handled by the built-in transitivity
  of the equivalence class representation:
  if there is a literal $x \xor \parity{1}$ for which
  $\True \equiv {x \xor \parity{1}}$ holds and
  the xor-clause $x \XX y \XX \parity{2}$ has been derived earlier,
  then $\True \equiv {y \xor (\parity{1} \xor \parity{2} \xor \True)}$
  as $\equiv$ also represents $x \XX y \XX \parity{2}$.
\item
  The \TerUnRule{} rule is applicable when
  (i) there are two variables, $x_1$ and $x_n$, such that
  $x_1 \equiv {x_n} \xor \parity{}'$ holds,
  and
  (ii) a xor-clause $x_1 \XX x_n \XX y \XX \parity{}$ in $\xorclauses$.

  When this rule is applied,
  (i) the equivalence classes of $\True$ and $y \xor \parity{}' \xor \parity{}$
  are merged, and
  (ii) the edge
  $\True \Bcgedge{\parity{}' \xor \parity{}}{x_1 \xor x_n \xor \parity{}' \xor \True} y$
  is added in the reason graph.
  %to record that $z \xor \parity{1} \xor \parity{2}$ has been derived because
  %$x_1$ is equivalent to ${x_n} \xor \parity{1}$.
\end{itemize}
In the following,
we only consider the sub-class of reason graphs producible by applying these rules.

\begin{example}
Consider again the formula $\xorclauses$ presented Ex.~\ref{ex:derivations} and compare the process below to the \ECsys-derivation discussed in the example. The initial equivalence relation $\equiv$ is the one representing $\xorclauses$, i.e. each literal in its own class. The full reason graph constructed is in Fig.~\ref{fig:eqgraph}: all shown edges are equality edges and ``@i'' annotation gives the index of the edge.

When we make the xor-assumption $a$, we first let $\equiv := \Merge{\equiv}{
\top}{a}$, find the xor-clause $(a \oplus b \oplus c) $ including $a$ in
    $\xorclauses$ and thus derive the xor-clause $ (b \oplus c \oplus \top)$ ,
    let $\equiv := \Merge{\equiv}{b}{c}$, and add the edge $ b \Bcgedge{\bot}{a}
    c$. We consider also the xor-clause $(a \oplus c \oplus d)$
    including $a$ in $\xorclauses$, derive the xor-clause 
 $ (c \oplus d \oplus \top)$, let $\equiv := \Merge{\equiv}{c}{d}$, and
 add the edge $ c \Bcgedge{\bot}{a} d$.  After this step,
we consider all clauses in $\xorclauses$ which include $b$ (or $d$, 
        the {\it smaller} equivalence class is preferred to avoid
        checking many clauses) whether they also include 
a variable from the equivalence class of $d$ ($b$ respectively).
Indeed, there is such a clause $(b \oplus d \oplus e) $ and
thus \TerUnRule{} rule is applicable, allowing us to derive the xor-implied literal $e$. The classes of $e$ and $\top$ are then merged; after this the equivalence relation is $\Set{\Set{\top,a,e},\Set{b,c,d}}$.
\end{example}

\begin{figure}
\centering
\includegraphics[width=.33\columnwidth]{eqgraph}
\caption{An equivalence reason graph}
\label{fig:eqgraph}
\end{figure}

\newcommand{\Expl}[1]{\alpha(#1)}
\newcommand{\ExplE}[1]{\beta(#1)}

If $x \xor \parity{}$ is a xor-implied literal,
then ${x \xor \parity{}} \equiv \True$
and
there is by construction a $\parity{}$-path
$\True \Bcgedge{\parity{1}}{r_1} z_1 \Bcgedge{\parity{2}}{r_2} z_2 ...
 z_k \Bcgedge{\parity{k}}{r_k} x$ in the graph
explaining why $x \xor \parity{}$ is implied.
%
To compute a xor-explanation for $x \xor \parity{}$,
we define a \emph{reason set} $\Expl{x \xor \parity{}}$ for it
%for $x \xor \parity{}$
to be a set of literals such that
$\Expl{x \xor \parity{}} =
 \ExplE{\True \Bcgedge{\parity{1}}{r_1} z_1} \cup
 \ExplE{z_1 \Bcgedge{\parity{2}}{r_2} z_2} \cup ... \cup
 \ExplE{z_k \Bcgedge{\parity{k}}{r_k} x}$ holds,
where each $\ExplE{v_1 \Bcgedge{\parity{}}{r} v_2}$ recursively
gives a reason for the edge $e = {v_1 \Bcgedge{\parity{}}{r} v_2}$ as follows:
\begin{itemize}
\item
  if $r = \Assump$ and $v_1 = \True$,
  then $\ExplE{e} = \Set{v_2 \xor \parity{}}$,
\item
  if $r$ is a unary clause $y \xor \parity{y}$,
  then $\ExplE{e} = \Expl{y \xor \parity{y}}$.
\item
  if $r$ is a binary clause $y \XX z \XX \parity{}'$,
  then $\ExplE{e} =
  \ExplE{y \Bcgedge{\parity{1}}{r_1} w_1} \cup
  \ExplE{w_1 {\Bcgedge{\parity{2}}{r_2}} w_2} \cup ... \cup
  \ExplE{w_k {\Bcgedge{\parity{k}}{r_k}} z}$
  for any $\parity{}'$-path
  $y {\Bcgedge{\parity{1}}{r_1}} w_1 {\Bcgedge{\parity{2}}{r_2}} ...
   w_k {\Bcgedge{\parity{k}}{r_k}} z$
  %with index less than that of $e$.
  having smaller index than $e$.
\end{itemize}

%
By construction
$\xorclauses \land (\bigwedge_{l \in \Expl{x \xor \parity{}}} l) \Models {x \xor \parity{}}$
and
thus a xor-explanation for $x \xor \parity{}$ is
$(x \xor \parity{}) \lor \bigvee_{l \in \Expl{x \xor \parity{}}} {\neg l}$.
%
\begin{example}
  Given the equivalence reason graph in Fig.~\ref{fig:eqgraph},
  the reason for $e$ is
  $\Expl{e} = \ExplE{\True \Bcgedge{\False}{b \xor d \xor \True} e} =
  \ExplE{b \Bcgedge{\False}{a} c} \cup
  \ExplE{c \Bcgedge{\False}{a} d} =
  \Expl{a} \cup \Expl{a} =
  \ExplE{\True \Bcgedge{\False}{\Assump} a} =
  \Set{a}$.
  Thus the xor-explanation for $e$ is
  $({\neg a} \lor e)$,
  corresponding to the ``cut 1'' in Fig.~\ref{ex:derivations}.
\hfill$\clubsuit$
\end{example}



==> resulttables.tex <==
\begin{figure}[ht]
\centering
\subfigure{
    \includegraphics[width=0.33\linewidth]{grain_time_median}
    \includegraphics[width=0.33\linewidth]{grain_decisions_median}
    \includegraphics[width=0.33\linewidth]{grain_propagations_median}
}
\subfigure{
    \includegraphics[width=0.33\linewidth]{hitag_time_median}
    \includegraphics[width=0.33\linewidth]{hitag_decisions_median}
    \includegraphics[width=0.33\linewidth]{hitag_propagations_median}
}
\subfigure{
    \includegraphics[width=0.33\linewidth]{trivium_time_median}
    \includegraphics[width=0.33\linewidth]{trivium_decisions_median}
    \includegraphics[width=0.33\linewidth]{trivium_propagations_median}
}
\caption{Medians of solving time, decisions, and propagations / decision}
\label{Fig:Results}
\end{figure}


==> substmodule.tex <==

%--------------------------------------------------------------------------
%
%--------------------------------------------------------------------------
%
%--------------------------------------------------------------------------
\section{The xor-reasoning module ``\ECAIsys{}''}
\label{Sect:ECAI}

This chapter introduces the necessary elements of the first xor-reasoning
module presented in~\cite{LJN:ECAI2010}. we refer it here as the ``\ECAIsys{}''
module because it is based on using substitution for propagating equivalence
information.
%
As explained above,
given a conjunction of xor-clauses $\xorclauses$ and
a sequence $l_1,...,l_k$ of xor-assumption literals,
the goal of the module is to deduce xor-implied literals and xor-conflicts
over $\xorclauses \land l_1 \land ... \land l_k$.
%
To do this,
the module implements a deduction system with the inference rules shown in
Fig.~\ref{fig:Rules},
each of the four rules consisting of two premises and one consequence.
%
The \unitrules{} rules perform unit propagation on xor-clauses while
the \eqvrules{} rules propagate equivalence information
(induced by binary xor-clauses)
on xor-clauses by substituting variable occurrences.

%
\begin{figure}[t]
  \centering
  \small
  \begin{tabular}{l@{\qquad}l}
    \unitruleP:\ 
    $\inferencerule{x}{C}{\simplification{C}{x}{\top}}$
    &
    \eqvruleP:\ 
    $\inferencerule{x_1 \oplus x_2 \oplus \True}{C}
    {\simplification{C}{x_1}{x_2}}$
    \\
    \\
    \unitruleN:\ 
    $\inferencerule{x \oplus \True}{C}{\simplification{C}{x}{\False}}$
    &
    \eqvruleN:\ 
    $\inferencerule{x_1 \oplus x_2}{C}
    {\simplification{C}{x_1}{(x_2\oplus\True)}}$
  \end{tabular}%
  \caption{Inference rules of \ECAIsys{}; the symbols $x$, $x_1$, and $x_2$ are variables while $C$ is a %(possibly empty)
xor-clause}
  \label{fig:Rules}%
  %\vspace{-4mm}
\end{figure}
%
If $\psi$ is a conjunction of xor-clauses,
a {\it \ECAIsys-derivation} on $\psi$
is a finite, vertex-labeled directed acyclic graph 
$\igraph = \Tuple{ \vertices, \edges, \Labfunc} $,
where each vertex $v \in \vertices$ is labeled with a xor-clause $\Lab{v}$ 
and
the following holds for each vertex $v$:
\begin{enumerate}
\item
  $v$ has no incoming edges (i.e.~is an \emph{input vertex})
  and
  $\Lab{v}$ is a xor-clause in $\psi$,
  or
  %$v$ is an input vertex and $\Lab{v}$ is a xor-clause in $\psi$, or
\item
  $v$ has two incoming edges,
  originating from vertices $v_1$ and $v_2$,
  and
  the xor-clause $\Lab{v}$ is derived from $ \Lab{v_1}$ and $\Lab{v_2}$
  by using one of the inference rules.
\end{enumerate}
%
A xor-clause $C$ is \emph{$\ECAIsys$-derivable} on $\psi$,
denoted by $\psi \ECAIderiv C$,
if there exists a xor-derivation on $\psi$ that contains a vertex
labeled with $C$;
the \ECAIsys-derivable unary xor-clauses are
the xor-implied literals that the \ECAIsys-module returns
when its \textsc{deduce} method is called.
%
As a direct consequence of the definition of xor-derivations and
the soundness of the inference rules,
it holds that if a xor-derivation on $\psi$ contains a vertex labeled
with the xor-clause $C$, then $C$ is a logical consequence of $\psi$,
i.e.~$\psi \ECAIderiv C$ implies $\psi \Conseq C$.
%
%As a direct consequence of the definition of xor-derivations and
%the soundness of the inference rules,
%it holds that if a xor-derivation on $\psi$ contains a vertex labeled
%with the xor-clause $C$, then $C$ is a logical consequence of $\psi$.
%%
%\begin{lemma}
%  $\psi \Deriv C$ implies $\psi \Conseq C$.
%  \label{Lemma:Deriv}
%\end{lemma}
%
A $\ECAIsys$-derivation on $\psi$ is a {\it $\ECAIsys$-refutation of $\psi$}
if it contains a vertex labeled with the false literal $\False$;
in this case, $\psi$ is unsatisfiable.
%
A $\ECAIsys$-derivation is {\it saturated} if it is not possible
to add a vertex with a new vertex label using the inference rules.
%
Note that $\ECAIsys$ is not refutationally complete,
e.g.~there is no $\ECAIsys$-refutation of the unsatisfiable conjunction
$(a \X b \X c) \land (a \X b \X c \X \True)$.
However, it is ``eventually refutationally complete'' in the DPLL(XOR) setting:
if each variable in $\psi$ occurs in a unary clause in $\psi$,
then the empty clause is $\ECAIsys$-derivable iff $\psi$ is unsatisfiable;
thus when the CDCL SAT solver has assigned a value to all variables in
$\xorclauses$,
the $\ECAIsys$-module can check whether all the xor-clauses are satisfied.


\iffalse
\begin{example}
  \label{Ex:ECAIa}
  Assume a conjunction of xor-clauses
  \begin{eqnarray*}
    \xorclauses &\!\!{=}\!\!&
    (a \X b \X c) \land
    (c \X d \X e) \land
    (b \X e \X f) \land
    \nonumber\\
    &&
    (e \X h \X i) \land
    (f \X g \X h) \land
    (b \X g \X i \XX {\True}).
  \end{eqnarray*}
  Figure~\ref{Fig:ECAI} shows
  an $\ECAIsys$-refutation of
  $\xorclauses \land (a) \land (d) \land (i)$;
  please ignore the node shapes and the ``cut'' lines for now.
  %
  The literal $f$ is $\ECAIsys$-derivable on $\xorclauses \land (a) \land (d)$;
  the $\ECAIsys$ xor-reasoning module returns
  $f$ as a xor-implied literal on $\xorclauses$ after
  $a$ and $d$ are given as xor-assumptions.
\hfill$\clubsuit$
\end{example}

\begin{figure}[h]
  \centering
  \includegraphics[width=.95\columnwidth]{ex-ecai3}
  \caption{A $\ECAIsys$-derivation}
  \label{Fig:ECAI}
\end{figure}

\fi


As explained in the previous section,
the CDCL part of the DPLL(XOR) framework requires an or-clause,
called xor-explanation, for each xor-implied literal.
%
These are computed by taking certain cuts in the derivation graph
$\igraph = \Tuple{ \vertices, \edges, \Labfunc} $. 
%
As usual, a \emph{cut} of $\igraph$ is a partitioning $(\VA,\VB)$ of
$\vertices$.
A \emph{cut for a non-input vertex $v \in \vertices$}
is a cut $(\VA,\VB)$ such that
(i) $v \in \VB$, and
(ii) if $v' \in \vertices$ is an input vertex and
there is a path from $v'$ to $v$, then $v' \in \VA$.
%
%A \emph{cut} for a non-input vertex $v \in \vertices$
%is a partitioning $(\VA,\VB)$ of $\vertices$ such that
%(i) $v \in \VB$, and
%(ii) if $v' \in \vertices$ is an input vertex and
%there is a path from $v'$ to $v$, then $v' \in \VA$.
%
The \emph{reason set} for a cut $\Cut=(\VA,\VB)$ is
$\RS{\Cut} = \Setdef{u \in \VA}{\exists u' \in \VB : \Tuple{u,u'} \in \edges}$.
%
As proven in \cite{LJN:ECAI2010},
it holds that if $W$ is a cut for $v$,
then $(\bigwedge_{u \in \RS{W}}\Lab{u}) \Models \Lab{v}$.
%
A cut $\Cut$ is \emph{cnf-compatible} if
for each $u \in \RS{\Cut}$ either
(i) $u$ is an input vertex, or
(ii) $\Lab{u}$ is a unary clause.
%
Given a conjunction $\xorclauses$ of xor-clauses,
xor-assumptions $l_1,...,l_k$,
and
a non-input vertex $v$ labeled with a literal $\IL$,
a xor-explanation of this xor-implied literal $\IL$ is
obtained by taking a cnf-compatible cut $\Cut$ for $v$
and
disjuncting the literal with the negations of the (unary) clauses in
$\Setdef{\Lab{u}}{{u \in \RS{\Cut}} \land {\Lab{u} \notin \xorclauses}}$.
%$\Setdef{u \in \RS{v}}{\Lab{u} \notin \xorclauses}$.
%



In the implementation used in \cite{LJN:ECAI2010}, the inference rules,
which are all of form
{\small $\inferencerule{A \oplus \alpha}{C}{\simplification{C}{A}{(\alpha \oplus \top)}}$},
are applied as rewriting rules modifying
the premise clause $C$ into $\simplification{C}{A}{(\alpha \oplus \top)}$.
%
\iffalse
As an example,
Fig.~\ref{Fig:ECAI} shows how the original xor-clauses in $\xorclauses$ of
Ex.~\ref{Ex:ECAIa} (illustrated with square boxes) are gradually rewritten
(to the ones shown with rounded, dashed boxes) when
the xor-assumptions $a$, $d$, and $i$ (with shaded rounded boxes) are made
one-by-one in that order.
\fi







